Node Compass: Multilevel Tracing and Debugging of Request Executions in JavaScript-Based Web-Servers

Adequate consideration is crucial to ensure that services in a distributed application context are running satisfactorily with the resources available. Due to the asynchronous nature of tasks and the need to work with multiple layers that deliver coordinated results in a single-threaded context, analysing performance is a challenging task in event-loop-based systems. The existing performance analysis methods for environments such as Node.js rely on higher-level instrumentation but lack precision, as they cannot capture the relevant underlying application flow. As a solution, we propose a streamlined method for recovering the asynchronous execution path of requests called the Nested Bounded Context Algorithm. The proposed technique tracks the application execution flow through multiple layers and showcases it on an interactive interface for further assessment. Furthermore, we introduce the vertical span concept. This representation of a span as a multidimensional object (horizontal and vertical) with a start and end of execution, along with its sub-layers and triggered operations, enables the granular identification and diagnosis of performance issues. We proposed a new technique called the Bounded Context Tracking Algorithm for event matching and request reassembling in a multi-layer trace . The two techniques allow aligning the executions of the request in a tree-based data structure for developed visualisations. These visualisations permit performance debugging of complex performance issues in Node.js.

==> name.tex <==
Advanced programming skills (C, C++, Java, Matlab, Perl, Python, C#, JSP, PHP)-
Mastering many distributions of Linux and Knowledge of UNIX plate-form
Very experienced in Cisco technologies such as Network IDS, eTrust AccessControl, Cisco Host-based IDS, ESM, and IDS, Catalyst, routers.
Proficient in SSL, web security architecture VPN, TCP/IP, IPSec , DNS, subversion,Paros, SpamAssassin, Nikto, Nmap and Nessus, TcpDump
Experienced in configuration, deployment and troubleshooting of high scale networks
Experienced in the security and deployment of many technology supportingprotocols such as Frame Relay, BGP, OSPF, EIGRP, DNS, POP3, SMTP, HTTP, VOIP,IPSec, FTP.
Experienced in writing Shell, Perl and Batch scripts for Server administration in Linux and Windows environments Advanced configuration and deployment skills of System services such as DNS,File Server, Web Sever, Firewall, Domain Controller
Experienced in penetration testing using tools such as Nessus, Metasploit

